Cuttlefish: Low-Rank Model Training without All the Tuning

Recent research has shown that training low-rank neural networks can effectively reduce the total number of trainable parameters without sacrificing predictive accuracy, resulting in end-to-end speedups. However, low-rank model training necessitates adjusting several additional factorization hyperparameters, such as the rank of the factorization at each layer. In this paper, we tackle this challenge by introducing Cuttlefish, an automated low-rank training approach that eliminates the need for tuning factorization hyperparameters. Cuttlefish leverages the observation that after a few epochs of full-rank training, the stable rank (i.e., an approximation of the true rank) of each layer stabilizes at a constant value. Cuttlefish switches from full-rank to low-rank training once the stable ranks of all layers have converged, setting the dimension of each factorization to its corresponding stable rank. Our results show that Cuttlefish generates models up to 5.6 times smaller than full-rank models, and attains up to a 1.2 times faster end-to-end training process while preserving comparable accuracy. Moreover, Cuttlefish outperforms state-of-the-art low-rank model training methods and other prominent baselines. The source code for our implementation can be found at: https://github.com/hwang595/Cuttlefish.

==> logo-latex-acm.tex <==
\usepackage[firstpage]{draftwatermark}
\SetWatermarkText{
 \hspace*{4.5in}
 \raisebox{9.5in}{
  \includegraphics[height=0.9in]{artifacts_available.pdf}
  \includegraphics[height=0.9in]{artifacts_evaluated_reusable.pdf}
 }
}
\SetWatermarkAngle{0}

